Meson modes of probe $D7$-branes in Klebanov-Strassler background

We examine the properties of 4-d bosonic and fermionic (mesons and mesinos) modes on $D7$-branes wrapped over Kuperstein 4-cycle of the Klebanov-Strassler background. The wave equations are derived in a convenient parameterization of the warped deformed conifold metric. The mass spectra, wave functions and couplings of bosonic modes are evaluated by means of semi-classical tools. We explore the possible existence of fermionic zero modes.

==> revstyle.tex <==
% fichier revstyle.tex 
\hfuzz =1pt
\overfullrule =0pt
\newcounter{subequation}[equation]
\makeatletter \fussy \flushbottom


\def \GUT { grand unified theories }
\def \wrt { with respect to }
\def \cft { conformal field theory }
\def \dof { degrees of freedom }
\def \bef { $\beta -$function }
\def \bet { beta function }
\def \mow { modular weights }
\def \loe { low energy }
\def \km { Kac-Moody }
\def \susy { supersymmetry }
\def \susyq { supersymmetric }
\def \sig { $\sigma -$model }
\def \ws { world sheet }
\def \tres { threshold corrections }
\def \L {\Lambda }
\def \l {\lambda } 
\def \ka {\kappa } 
\def \t {\theta }
\def \vt {\vartheta }
\def \T {\Theta }
\def \vT {\hat {\vartheta } }
\def \a {\alpha }
\def \dh {\partial }
\def \d {\delta }
\def \D {\Delta }
\def \bq {\bar q }
\def \bQ {\bar Q}
\def \g {\gamma }
\def \G {\Gamma }
\def \O {\Omega }
\def \o {\omega }
\def \b {\beta }
\def \S {\Sigma }
\def \s {\sigma }
\def \e {\epsilon }
\def \cc { coupling constant }
\def \ccs {coupling constants }
\def \ph { phenomenology } 
\def \pheny { phenomenologically } 
\def \rhs { right hand side } 
\def \lhs {left  hand side } 
\def \ren { renormalization } 
\def \rge { renormalization group equations}
\def \ud { {1 \over 2} } 
\def \ut { {1 \over 3} } 
\def \td {{3 \over  2 }} 
\def \sm { standard model }
\def \q {\eqno  }
\def \mssm { minimal supersymmetric standard model } 
\def \he  { high energy }
\def \st { string theory }
\def \ft { field theory }
\def \cddd { {\cal D } }
\def \cala { {\cal A } }
\def \calc { {\cal C } }
\def \calp { {\cal P } }
\def \caly { {\cal Y } }
\def \calf { {\cal F } }
\def \calg { {\cal G } }
\def \calq { {\cal Q } }
\def \caln { {\cal N } }
\def \call { {\cal L } }
\def \cale { {\cal E } }
\def \calG { {\cal G } }
\def \calH { {\cal H } }
\def \calk { {\cal K } }
\def \calt { {\Theta } }
\def \calT { {\cal T } }
\def \cald { {\cal D } }
\def \cali { {\cal I } }
\def \calj { {\cal J } }
\def \calb { {\cal B } }
\def \calm { {\cal M } }
\def \calr { {\cal R } }
\def \cals { {\cal S } }
\def \calu { {\cal U } }
\def \calo { {\cal O } }
\def \calz { {\cal z } }
\def \cals { {\cal S } }
\def \calv { {\cal V } }
\def \calw { {\cal W } }
\def \calx { {\cal X } }
\def \calY { {\cal Y } }
\def \ua  {\underline {a}}
\def \uA  {\underline {A}}
\def \ub  {\underline {b}}
\def \uc  {\underline {c}}
\def \udd  {\underline {d}}
\def \ul  {\underline {l}}
\def \um  {\underline {m}}
\def \uM  {\underline {M}}
\def \un  {\underline {n}}
\def \uA  {\underline {A}}
\def \uB  {\underline {B}}
\def \umg  {\underline {\mu }}
\def \ung  {\underline {\nu }}
\def \ui  {\underline { i }}
\def \uj  {\underline {j}}
\def \uag  {\underline {\alpha }}
\def \ubg  {\underline {\beta }}
\def \ugg  {\underline {\gamma }}
\def \udg  {\underline {\delta }}
\def  \bR  {\textbf  {R}}
\def  \bC   {\textbf{C}}
%\def \bea {\begin{equation}}
%\def \eea {\end{equation}}
\def \tchi  {{\tilde \chi }}
\def \Eslash {E \kern-.5em\slash}
\def \epslash {\epsilon \kern-.5em\slash}
\def \pslash {p \kern-.5em\slash}
\def \kslash {k \kern-.5em\slash}
\def \Dslash {D \kern-.5em\slash}
\def \Hslash {H \kern-.5em\slash}
\def \dslash {\partial \kern-.5em\slash}
\def \vslash {v \kern-.5em\slash}
\def \Gslash {G \kern-.5em\slash}
\def \Hslash {H \kern-.5em\slash}
\def \Fslash {F \kern-.5em\slash}
\def \oslash {o \kern-.5em\slash}
\def \Pslash {P \kern-.5em\slash}
\def \slashf {{\cal F}  \kern-.5em\slash}
\def \bull {$\bullet  \quad $}
\def \bfA { {\bf A} }
\def \bfB { {\bf B} }
\def \bfS { {\bf S} }
\def \jmp { Jour. Math. Phys. }
\def \ptp { Prog. Theor. Phys. }
\def \ap {Ann. Phys. (NY) }
\def \z {Z. Phys. } 
\def \pr  { Phys. Rev. }
\def \np { Nucl. Phys. }  
\def \arr { Ann. Rev. Nucl. Sci. } 
\def \ar { Ann. Rev. Nucl. Part. Sci. } 
\def \pp { Phys. Reports } 
\def \je { Sov. Phys. JETP } 
\def \prl { Phys. Rev. Lett. } 
\def \pl { Phys. Lett. }
\def \rmp { Rev. Mod. Phys. } 
\def \nc { Nuovo Cimento }
\def \jnp { Sov. Jour. Nucl. Phys. }
\def\NPB#1#2#3 {{\rm Nucl.~Phys.}  {\bf{B#1}}, {#3} (#2)}
\def\NPA#1#2#3 {{\rm Nucl.~Phys.}  {\bf{A#1}}, {#3} (#2)}
\def\PLB#1#2#3 {{\rm Phys.~Lett.}  {\bf{B#1}}, {#3} (#2)}
\def\PR#1#2#3 {{\rm Phys.~Rep.}  {\bf#1}, {#3} (#2)} 
\def\PRD#1#2#3 {{\rm Phys.~Rev.}  {\bf{D#1}}, {#3} (#2)} 
\def\PRL#1#2#3  {{\rm Phys.~Rev.~Lett.}  {\bf{#1}}, {#3} (#2)} 
\def\ZPC#1#2#3 {{\rm Z.~Phys.}  {\bf C#1}, {#3} (#2)} 
\def\JHEP#1#2#3 {{\rm JHEP} {\bf C#1}, {#3}  (#2)}     
\def\IJMP#1#2#3 {{\rm Int. J. Mod. Phys.}  {\bf A#1}, {#3} (#2)} 
\def\JMP#1#2#3 {{\rm J. Math. Phys.}  {\bf #1}, {#3} (#2)}
\def\PTP#1#2#3 {{\rm Prog. Theor. Phys.}  {\bf{#1}}, {#3} (#2)}
\def\FP#1#2#3  {{\rm  Fortsch. Phys.}  {\bf{#1}}, {#3} (#2)}
\def\CMP#1#2#3  {{\rm Comm. Math. Phys.}  {\bf{#1}}, {#3} (#2)}
\def\RMP#1#2#3  {{\rm Rev.  Mod. Phys.}  {\bf{#1}}, {#3} (#2)}

%%%%%%RICCI PACKAGE %%%%%%%%%%%%%
\def\mysavedown#1{\edef\mysubs{\mysubs#1}}
\def\mysaveup#1{\edef\mysups{\mysups#1}}
\def\mydown#1{{\mytensor}_{\vphantom{\mysubs}#1}}
\def\myup#1{{\mytensor}^{\vphantom{\mysups}#1}}
\def\tensor#1#2{
  #1
  \def\mytensor{\vphantom{#1}}
  \def\mysubs{\relax}
  \def\mysups{\relax}
% Make one pass across indices to determine maximum height.
  \let\down=\mysavedown
  \let\up=\mysaveup
  #2
% Now make a second pass to typeset the sub- & superscripts.
  \let\down=\mydown
  \let\up=\myup
  #2
  }
\def\Alt{\mathop{\hbox{Alt}}\nolimits}
\def\Sym{\mathop{\hbox{Sym}}\nolimits}
\def\Del{\mathop\nabla\nolimits}
\def\grad{\mathop{\hbox{grad}}\nolimits}
\def\div{\mathop{\hbox{div}}\nolimits}
\def\extd{\mathop{d}\nolimits}
\def\Lie{\cal L} 
%% Change this to "\Cal L" for amstex

%\rightline {hep-th/}
%\rightline  {T98/}
%\hoffset-1in
%\voffset-1in
%\if@twoside\oddsidemargin15mm
%\evensidemargin15mm\marginparwidth15mm
%\else\oddsidemargin15mm\evensidemargin15mm\marginparwidth15mm\fi
%\footheight12pt\footskip30pt
%\textwidth 18 cm
%\baselineskip15pt
%\textheight 45\baselineskip
%\makeatletter
%Subequations

\def\thesubequation{\theequation\@alph\c@subequation}
\def\@subeqnnum{{\rm (\thesubequation)}}
\def\slabel#1{\@bsphack\if@filesw {\let\thepage\relax
   \xdef\@gtempa{\write\@auxout{\string
      \newlabel{#1}{{\thesubequation}{\thepage}}}}}\@gtempa
   \if@nobreak \ifvmode\nobreak\fi\fi\fi\@esphack}
\def\subeqnarray{\stepcounter{equation}
\let\@currentlabel=\theequation\global\c@subequation\@ne
\global\@eqnswtrue
\global\@eqcnt\z@\tabskip\@centering\let\\=\@subeqncr
$$\halign to \displaywidth\bgroup\@eqnsel\hskip\@centering
  $\displaystyle\tabskip\z@{##}$&\global\@eqcnt\@ne
  \hskip 2\arraycolsep \hfil${##}$\hfil
  &\global\@eqcnt\tw@ \hskip 2\arraycolsep
  $\displaystyle\tabskip\z@{##}$\hfil
   \tabskip\@centering&\llap{##}\tabskip\z@\cr}
\def\endsubeqnarray{\@@subeqncr\egroup
                     $$\global\@ignoretrue}
\def\@subeqncr{{\ifnum0=`}\fi\@ifstar{\global\@eqpen\@M
    \@ysubeqncr}{\global\@eqpen\interdisplaylinepenalty \@ysubeqncr}}
\def\@ysubeqncr{\@ifnextchar [{\@xsubeqncr}{\@xsubeqncr[\z@]}}
\def\@xsubeqncr[#1]{\ifnum0=`{\fi}\@@subeqncr
   \noalign{\penalty\@eqpen\vskip\jot\vskip #1\relax}}
\def\@@subeqncr{\let\@tempa\relax
    \ifcase\@eqcnt \def\@tempa{& & &}\or \def\@tempa{& &}
      \else \def\@tempa{&}\fi
     \@tempa \if@eqnsw\@subeqnnum\refstepcounter{subequation}\fi
     \global\@eqnswtrue\global\@eqcnt\z@\cr}
\let\@ssubeqncr=\@subeqncr
\@namedef{subeqnarray*}{\def\@subeqncr{\nonumber\@ssubeqncr}\subeqnarray}
\@namedef{endsubeqnarray*}{\global\advance\c@equation\m@ne%
                           \nonumber\endsubeqnarray}


%Number equations by section
\@addtoreset{equation}{section}
\renewcommand{\theequation}{\thesection.\arabic{equation}}
%Other macros
%\newcommand{\bm}{\bibitem}
\newcommand{\be}{\begin{equation}} 
\newcommand{\ee}{\end{equation}} 
\newcommand{\ba}{\begin{array}}
\newcommand{\ea}{\end{array}}
\newcommand{\bea}{\begin{eqnarray}} 
\newcommand{\eea}{\end{eqnarray}} 
\newcommand{\bsea}{\begin{subeqnarray}} 
\newcommand{\esea}{\end{subeqnarray}}
\newcommand{\nn}{\nonumber}






